A Bias-Variance Decomposition for Ensembles over Multiple Synthetic Datasets

Recent studies have highlighted the benefits of generating multiple synthetic datasets for supervised learning, from increased accuracy to more effective model selection and uncertainty estimation. These benefits have clear empirical support, but the theoretical understanding of them is currently very light. We seek to increase the theoretical understanding by deriving bias-variance decompositions for several settings of using multiple synthetic datasets, including differentially private synthetic data. Our theory yields a simple rule of thumb to select the appropriate number of synthetic datasets in the case of mean-squared error and Brier score. We investigate how our theory works in practice with several real datasets, downstream predictors and error metrics. As our theory predicts, multiple synthetic datasets often improve accuracy, while a single large synthetic dataset gives at best minimal improvement, showing that our insights are practically relevant.

==> figures/classification/adult-mse-est-table.tex <==
\begin{tabular}{lllllllll}
\toprule
 &  & m & 1 & 2 & 4 & 8 & 16 & 32 \\
Downstream & Generator & Predicted / Measured &  &  &  &  &  &  \\
\midrule
\multirow[c]{4}{*}{1-NN} & \multirow[c]{2}{*}{DDPM} & Measured & 0.24 $\pm$ 0.004 & 0.19 $\pm$ 0.004 & 0.17 $\pm$ 0.015 & 0.17 $\pm$ 0.019 & 0.16 $\pm$ 0.019 & 0.16 $\pm$ 0.020 \\
 &  & Predicted & 0.24 $\pm$ 0.004 & 0.19 $\pm$ 0.004 & 0.16 $\pm$ 0.005 & 0.15 $\pm$ 0.005 & 0.14 $\pm$ 0.006 & 0.14 $\pm$ 0.006 \\
\cline{2-9}
 & \multirow[c]{2}{*}{SP-P} & Measured & 0.21 $\pm$ 0.005 & 0.16 $\pm$ 0.003 & 0.14 $\pm$ 0.012 & 0.13 $\pm$ 0.015 & 0.13 $\pm$ 0.015 & 0.12 $\pm$ 0.014 \\
 &  & Predicted & 0.21 $\pm$ 0.005 & 0.16 $\pm$ 0.003 & 0.13 $\pm$ 0.002 & 0.12 $\pm$ 0.003 & 0.11 $\pm$ 0.003 & 0.11 $\pm$ 0.003 \\
\cline{1-9} \cline{2-9}
\multirow[c]{4}{*}{5-NN} & \multirow[c]{2}{*}{DDPM} & Measured & 0.14 $\pm$ 0.003 & 0.14 $\pm$ 0.003 & 0.13 $\pm$ 0.005 & 0.13 $\pm$ 0.005 & 0.13 $\pm$ 0.005 & 0.13 $\pm$ 0.004 \\
 &  & Predicted & 0.14 $\pm$ 0.003 & 0.14 $\pm$ 0.003 & 0.13 $\pm$ 0.004 & 0.13 $\pm$ 0.005 & 0.13 $\pm$ 0.005 & 0.13 $\pm$ 0.006 \\
\cline{2-9}
 & \multirow[c]{2}{*}{SP-P} & Measured & 0.14 $\pm$ 0.003 & 0.13 $\pm$ 0.007 & 0.13 $\pm$ 0.010 & 0.12 $\pm$ 0.010 & 0.12 $\pm$ 0.009 & 0.12 $\pm$ 0.009 \\
 &  & Predicted & 0.14 $\pm$ 0.003 & 0.13 $\pm$ 0.007 & 0.13 $\pm$ 0.011 & 0.12 $\pm$ 0.012 & 0.12 $\pm$ 0.013 & 0.12 $\pm$ 0.013 \\
\cline{1-9} \cline{2-9}
\multirow[c]{4}{*}{Decision Tree} & \multirow[c]{2}{*}{DDPM} & Measured & 0.21 $\pm$ 0.000 & 0.17 $\pm$ 0.004 & 0.15 $\pm$ 0.014 & 0.14 $\pm$ 0.015 & 0.13 $\pm$ 0.015 & 0.13 $\pm$ 0.014 \\
 &  & Predicted & 0.21 $\pm$ 0.000 & 0.17 $\pm$ 0.004 & 0.14 $\pm$ 0.006 & 0.13 $\pm$ 0.007 & 0.12 $\pm$ 0.007 & 0.12 $\pm$ 0.008 \\
\cline{2-9}
 & \multirow[c]{2}{*}{SP-P} & Measured & 0.18 $\pm$ 0.002 & 0.14 $\pm$ 0.005 & 0.13 $\pm$ 0.012 & 0.12 $\pm$ 0.012 & 0.11 $\pm$ 0.011 & 0.11 $\pm$ 0.011 \\
 &  & Predicted & 0.18 $\pm$ 0.002 & 0.14 $\pm$ 0.005 & 0.12 $\pm$ 0.008 & 0.12 $\pm$ 0.009 & 0.11 $\pm$ 0.010 & 0.11 $\pm$ 0.010 \\
\cline{1-9} \cline{2-9}
\multirow[c]{4}{*}{Random Forest} & \multirow[c]{2}{*}{DDPM} & Measured & 0.12 $\pm$ 0.001 & 0.12 $\pm$ 0.001 & 0.11 $\pm$ 0.001 & 0.11 $\pm$ 0.001 & 0.11 $\pm$ 0.001 & 0.11 $\pm$ 0.001 \\
 &  & Predicted & 0.12 $\pm$ 0.001 & 0.12 $\pm$ 0.001 & 0.11 $\pm$ 0.001 & 0.11 $\pm$ 0.001 & 0.11 $\pm$ 0.001 & 0.11 $\pm$ 0.001 \\
\cline{2-9}
 & \multirow[c]{2}{*}{SP-P} & Measured & 0.12 $\pm$ 0.002 & 0.11 $\pm$ 0.002 & 0.10 $\pm$ 0.003 & 0.10 $\pm$ 0.002 & 0.10 $\pm$ 0.002 & 0.10 $\pm$ 0.002 \\
 &  & Predicted & 0.12 $\pm$ 0.002 & 0.11 $\pm$ 0.002 & 0.10 $\pm$ 0.003 & 0.10 $\pm$ 0.003 & 0.10 $\pm$ 0.003 & 0.10 $\pm$ 0.003 \\
\cline{1-9} \cline{2-9}
\multirow[c]{4}{*}{MLP} & \multirow[c]{2}{*}{DDPM} & Measured & 0.14 $\pm$ 0.005 & 0.13 $\pm$ 0.002 & 0.12 $\pm$ 0.002 & 0.12 $\pm$ 0.002 & 0.11 $\pm$ 0.002 & 0.11 $\pm$ 0.002 \\
 &  & Predicted & 0.14 $\pm$ 0.005 & 0.13 $\pm$ 0.002 & 0.12 $\pm$ 0.003 & 0.12 $\pm$ 0.004 & 0.12 $\pm$ 0.004 & 0.12 $\pm$ 0.005 \\
\cline{2-9}
 & \multirow[c]{2}{*}{SP-P} & Measured & 0.13 $\pm$ 0.003 & 0.12 $\pm$ 0.002 & 0.11 $\pm$ 0.002 & 0.11 $\pm$ 0.002 & 0.10 $\pm$ 0.003 & 0.10 $\pm$ 0.002 \\
 &  & Predicted & 0.13 $\pm$ 0.003 & 0.12 $\pm$ 0.002 & 0.11 $\pm$ 0.002 & 0.11 $\pm$ 0.002 & 0.10 $\pm$ 0.002 & 0.10 $\pm$ 0.002 \\
\cline{1-9} \cline{2-9}
\multirow[c]{4}{*}{Gradient Boosting} & \multirow[c]{2}{*}{DDPM} & Measured & 0.11 $\pm$ 0.002 & 0.11 $\pm$ 0.000 & 0.11 $\pm$ 0.000 & 0.11 $\pm$ 0.000 & 0.11 $\pm$ 0.000 & 0.11 $\pm$ 0.001 \\
 &  & Predicted & 0.11 $\pm$ 0.002 & 0.11 $\pm$ 0.000 & 0.11 $\pm$ 0.000 & 0.11 $\pm$ 0.001 & 0.11 $\pm$ 0.001 & 0.11 $\pm$ 0.001 \\
\cline{2-9}
 & \multirow[c]{2}{*}{SP-P} & Measured & 0.10 $\pm$ 0.001 & 0.10 $\pm$ 0.001 & 0.10 $\pm$ 0.001 & 0.10 $\pm$ 0.001 & 0.10 $\pm$ 0.001 & 0.10 $\pm$ 0.001 \\
 &  & Predicted & 0.10 $\pm$ 0.001 & 0.10 $\pm$ 0.001 & 0.10 $\pm$ 0.001 & 0.10 $\pm$ 0.001 & 0.10 $\pm$ 0.001 & 0.10 $\pm$ 0.001 \\
\cline{1-9} \cline{2-9}
\multirow[c]{4}{*}{SVM} & \multirow[c]{2}{*}{DDPM} & Measured & 0.12 $\pm$ 0.002 & 0.12 $\pm$ 0.001 & 0.12 $\pm$ 0.000 & 0.12 $\pm$ 0.000 & 0.12 $\pm$ 0.000 & 0.12 $\pm$ 0.000 \\
 &  & Predicted & 0.12 $\pm$ 0.002 & 0.12 $\pm$ 0.001 & 0.12 $\pm$ 0.002 & 0.12 $\pm$ 0.002 & 0.12 $\pm$ 0.002 & 0.12 $\pm$ 0.002 \\
\cline{2-9}
 & \multirow[c]{2}{*}{SP-P} & Measured & 0.12 $\pm$ 0.001 & 0.11 $\pm$ 0.001 & 0.11 $\pm$ 0.001 & 0.11 $\pm$ 0.001 & 0.11 $\pm$ 0.001 & 0.11 $\pm$ 0.001 \\
 &  & Predicted & 0.12 $\pm$ 0.001 & 0.11 $\pm$ 0.001 & 0.11 $\pm$ 0.001 & 0.11 $\pm$ 0.001 & 0.11 $\pm$ 0.001 & 0.11 $\pm$ 0.001 \\
\cline{1-9} \cline{2-9}
\multirow[c]{4}{*}{Logistic Regression} & \multirow[c]{2}{*}{DDPM} & Measured & 0.12 $\pm$ 0.001 & 0.11 $\pm$ 0.002 & 0.12 $\pm$ 0.001 & 0.11 $\pm$ 0.001 & 0.11 $\pm$ 0.000 & 0.11 $\pm$ 0.000 \\
 &  & Predicted & 0.12 $\pm$ 0.001 & 0.11 $\pm$ 0.002 & 0.11 $\pm$ 0.003 & 0.11 $\pm$ 0.004 & 0.11 $\pm$ 0.004 & 0.11 $\pm$ 0.004 \\
\cline{2-9}
 & \multirow[c]{2}{*}{SP-P} & Measured & 0.10 $\pm$ 0.001 & 0.10 $\pm$ 0.001 & 0.10 $\pm$ 0.001 & 0.10 $\pm$ 0.001 & 0.10 $\pm$ 0.001 & 0.10 $\pm$ 0.001 \\
 &  & Predicted & 0.10 $\pm$ 0.001 & 0.10 $\pm$ 0.001 & 0.10 $\pm$ 0.001 & 0.10 $\pm$ 0.001 & 0.10 $\pm$ 0.001 & 0.10 $\pm$ 0.001 \\
\cline{1-9} \cline{2-9}
\bottomrule
\end{tabular}


==> figures/classification/breast-cancer-mse-est-table.tex <==
\begin{tabular}{lllllllll}
\toprule
 &  & m & 1 & 2 & 4 & 8 & 16 & 32 \\
Downstream & Generator & Predicted / Measured &  &  &  &  &  &  \\
\midrule
\multirow[c]{4}{*}{1-NN} & \multirow[c]{2}{*}{DDPM} & Measured & 0.12 $\pm$ 0.067 & 0.09 $\pm$ 0.048 & 0.09 $\pm$ 0.048 & 0.10 $\pm$ 0.041 & 0.10 $\pm$ 0.041 & 0.10 $\pm$ 0.040 \\
 &  & Predicted & 0.12 $\pm$ 0.067 & 0.09 $\pm$ 0.048 & 0.08 $\pm$ 0.049 & 0.07 $\pm$ 0.052 & 0.07 $\pm$ 0.054 & 0.07 $\pm$ 0.056 \\
\cline{2-9}
 & \multirow[c]{2}{*}{SP-P} & Measured & 0.11 $\pm$ 0.041 & 0.07 $\pm$ 0.014 & 0.05 $\pm$ 0.011 & 0.04 $\pm$ 0.003 & 0.04 $\pm$ 0.002 & 0.03 $\pm$ 0.002 \\
 &  & Predicted & 0.11 $\pm$ 0.041 & 0.07 $\pm$ 0.014 & 0.04 $\pm$ 0.010 & 0.03 $\pm$ 0.014 & 0.03 $\pm$ 0.018 & 0.03 $\pm$ 0.019 \\
\cline{1-9} \cline{2-9}
\multirow[c]{4}{*}{5-NN} & \multirow[c]{2}{*}{DDPM} & Measured & 0.14 $\pm$ 0.077 & 0.13 $\pm$ 0.070 & 0.13 $\pm$ 0.070 & 0.12 $\pm$ 0.065 & 0.12 $\pm$ 0.058 & 0.12 $\pm$ 0.062 \\
 &  & Predicted & 0.14 $\pm$ 0.077 & 0.13 $\pm$ 0.070 & 0.12 $\pm$ 0.068 & 0.11 $\pm$ 0.068 & 0.11 $\pm$ 0.068 & 0.11 $\pm$ 0.068 \\
\cline{2-9}
 & \multirow[c]{2}{*}{SP-P} & Measured & 0.05 $\pm$ 0.011 & 0.04 $\pm$ 0.004 & 0.04 $\pm$ 0.005 & 0.03 $\pm$ 0.003 & 0.03 $\pm$ 0.004 & 0.03 $\pm$ 0.004 \\
 &  & Predicted & 0.05 $\pm$ 0.011 & 0.04 $\pm$ 0.004 & 0.03 $\pm$ 0.003 & 0.03 $\pm$ 0.004 & 0.03 $\pm$ 0.005 & 0.03 $\pm$ 0.006 \\
\cline{1-9} \cline{2-9}
\multirow[c]{4}{*}{Decision Tree} & \multirow[c]{2}{*}{DDPM} & Measured & 0.14 $\pm$ 0.074 & 0.09 $\pm$ 0.023 & 0.09 $\pm$ 0.023 & 0.09 $\pm$ 0.026 & 0.09 $\pm$ 0.027 & 0.09 $\pm$ 0.025 \\
 &  & Predicted & 0.14 $\pm$ 0.074 & 0.09 $\pm$ 0.023 & 0.06 $\pm$ 0.022 & 0.05 $\pm$ 0.033 & 0.04 $\pm$ 0.039 & 0.04 $\pm$ 0.042 \\
\cline{2-9}
 & \multirow[c]{2}{*}{SP-P} & Measured & 0.10 $\pm$ 0.025 & 0.05 $\pm$ 0.011 & 0.04 $\pm$ 0.007 & 0.03 $\pm$ 0.004 & 0.03 $\pm$ 0.007 & 0.03 $\pm$ 0.004 \\
 &  & Predicted & 0.10 $\pm$ 0.025 & 0.05 $\pm$ 0.011 & 0.03 $\pm$ 0.005 & 0.02 $\pm$ 0.004 & 0.01 $\pm$ 0.005 & 0.01 $\pm$ 0.006 \\
\cline{1-9} \cline{2-9}
\multirow[c]{4}{*}{Random Forest} & \multirow[c]{2}{*}{DDPM} & Measured & 0.08 $\pm$ 0.030 & 0.07 $\pm$ 0.016 & 0.07 $\pm$ 0.017 & 0.07 $\pm$ 0.017 & 0.07 $\pm$ 0.020 & 0.07 $\pm$ 0.020 \\
 &  & Predicted & 0.08 $\pm$ 0.030 & 0.07 $\pm$ 0.016 & 0.06 $\pm$ 0.015 & 0.06 $\pm$ 0.016 & 0.06 $\pm$ 0.018 & 0.06 $\pm$ 0.018 \\
\cline{2-9}
 & \multirow[c]{2}{*}{SP-P} & Measured & 0.04 $\pm$ 0.003 & 0.03 $\pm$ 0.007 & 0.03 $\pm$ 0.007 & 0.03 $\pm$ 0.006 & 0.03 $\pm$ 0.006 & 0.03 $\pm$ 0.006 \\
 &  & Predicted & 0.04 $\pm$ 0.003 & 0.03 $\pm$ 0.007 & 0.03 $\pm$ 0.009 & 0.03 $\pm$ 0.011 & 0.03 $\pm$ 0.011 & 0.03 $\pm$ 0.011 \\
\cline{1-9} \cline{2-9}
\multirow[c]{4}{*}{MLP} & \multirow[c]{2}{*}{DDPM} & Measured & 0.05 $\pm$ 0.014 & 0.05 $\pm$ 0.007 & 0.04 $\pm$ 0.006 & 0.05 $\pm$ 0.009 & 0.05 $\pm$ 0.014 & 0.05 $\pm$ 0.015 \\
 &  & Predicted & 0.05 $\pm$ 0.014 & 0.05 $\pm$ 0.007 & 0.04 $\pm$ 0.012 & 0.04 $\pm$ 0.016 & 0.04 $\pm$ 0.018 & 0.04 $\pm$ 0.019 \\
\cline{2-9}
 & \multirow[c]{2}{*}{SP-P} & Measured & 0.05 $\pm$ 0.011 & 0.04 $\pm$ 0.009 & 0.03 $\pm$ 0.004 & 0.03 $\pm$ 0.001 & 0.03 $\pm$ 0.005 & 0.02 $\pm$ 0.004 \\
 &  & Predicted & 0.05 $\pm$ 0.011 & 0.04 $\pm$ 0.009 & 0.04 $\pm$ 0.008 & 0.04 $\pm$ 0.008 & 0.04 $\pm$ 0.008 & 0.04 $\pm$ 0.008 \\
\cline{1-9} \cline{2-9}
\multirow[c]{4}{*}{Gradient Boosting} & \multirow[c]{2}{*}{DDPM} & Measured & 0.13 $\pm$ 0.080 & 0.09 $\pm$ 0.028 & 0.09 $\pm$ 0.030 & 0.08 $\pm$ 0.026 & 0.08 $\pm$ 0.029 & 0.08 $\pm$ 0.028 \\
 &  & Predicted & 0.13 $\pm$ 0.080 & 0.09 $\pm$ 0.028 & 0.06 $\pm$ 0.028 & 0.05 $\pm$ 0.038 & 0.05 $\pm$ 0.045 & 0.04 $\pm$ 0.048 \\
\cline{2-9}
 & \multirow[c]{2}{*}{SP-P} & Measured & 0.04 $\pm$ 0.002 & 0.04 $\pm$ 0.003 & 0.03 $\pm$ 0.002 & 0.03 $\pm$ 0.003 & 0.03 $\pm$ 0.005 & 0.03 $\pm$ 0.005 \\
 &  & Predicted & 0.04 $\pm$ 0.002 & 0.04 $\pm$ 0.003 & 0.03 $\pm$ 0.006 & 0.03 $\pm$ 0.007 & 0.03 $\pm$ 0.008 & 0.03 $\pm$ 0.008 \\
\cline{1-9} \cline{2-9}
\multirow[c]{4}{*}{SVM} & \multirow[c]{2}{*}{DDPM} & Measured & 0.11 $\pm$ 0.045 & 0.11 $\pm$ 0.047 & 0.11 $\pm$ 0.047 & 0.11 $\pm$ 0.048 & 0.11 $\pm$ 0.046 & 0.11 $\pm$ 0.046 \\
 &  & Predicted & 0.11 $\pm$ 0.045 & 0.11 $\pm$ 0.047 & 0.11 $\pm$ 0.048 & 0.11 $\pm$ 0.049 & 0.11 $\pm$ 0.049 & 0.11 $\pm$ 0.049 \\
\cline{2-9}
 & \multirow[c]{2}{*}{SP-P} & Measured & 0.04 $\pm$ 0.005 & 0.04 $\pm$ 0.006 & 0.03 $\pm$ 0.004 & 0.03 $\pm$ 0.003 & 0.03 $\pm$ 0.003 & 0.03 $\pm$ 0.003 \\
 &  & Predicted & 0.04 $\pm$ 0.005 & 0.04 $\pm$ 0.006 & 0.04 $\pm$ 0.008 & 0.04 $\pm$ 0.008 & 0.04 $\pm$ 0.009 & 0.04 $\pm$ 0.009 \\
\cline{1-9} \cline{2-9}
\multirow[c]{4}{*}{Logistic Regression} & \multirow[c]{2}{*}{DDPM} & Measured & 0.11 $\pm$ 0.050 & 0.10 $\pm$ 0.063 & 0.10 $\pm$ 0.063 & 0.09 $\pm$ 0.067 & 0.10 $\pm$ 0.069 & 0.10 $\pm$ 0.069 \\
 &  & Predicted & 0.11 $\pm$ 0.050 & 0.10 $\pm$ 0.063 & 0.09 $\pm$ 0.069 & 0.09 $\pm$ 0.072 & 0.08 $\pm$ 0.073 & 0.08 $\pm$ 0.074 \\
\cline{2-9}
 & \multirow[c]{2}{*}{SP-P} & Measured & 0.04 $\pm$ 0.008 & 0.03 $\pm$ 0.003 & 0.03 $\pm$ 0.003 & 0.03 $\pm$ 0.003 & 0.02 $\pm$ 0.004 & 0.02 $\pm$ 0.004 \\
 &  & Predicted & 0.04 $\pm$ 0.008 & 0.03 $\pm$ 0.003 & 0.03 $\pm$ 0.008 & 0.03 $\pm$ 0.011 & 0.03 $\pm$ 0.012 & 0.03 $\pm$ 0.013 \\
\cline{1-9} \cline{2-9}
\bottomrule
\end{tabular}


==> figures/regression/abalone-mse-est-table.tex <==
\begin{tabular}{lllllllll}
\toprule
 &  & m & 1 & 2 & 4 & 8 & 16 & 32 \\
Downstream & Generator & Predicted / Measured &  &  &  &  &  &  \\
\midrule
\multirow[c]{4}{*}{Linear Regression} & \multirow[c]{2}{*}{DDPM} & Predicted & 8.24 $\pm$ 2.392 & 8.24 $\pm$ 2.392 & 8.24 $\pm$ 2.392 & 8.24 $\pm$ 2.392 & 8.24 $\pm$ 2.392 & 8.24 $\pm$ 2.392 \\
 &  & Measured & 8.24 $\pm$ 2.392 & 8.24 $\pm$ 2.392 & 8.31 $\pm$ 2.334 & 8.25 $\pm$ 2.388 & 7.79 $\pm$ 1.602 & 7.79 $\pm$ 1.602 \\
\cline{2-9}
 & \multirow[c]{2}{*}{SP-P} & Predicted & 5.57 $\pm$ 0.646 & 5.42 $\pm$ 0.429 & 5.35 $\pm$ 0.352 & 5.31 $\pm$ 0.328 & 5.29 $\pm$ 0.321 & 5.28 $\pm$ 0.319 \\
 &  & Measured & 5.57 $\pm$ 0.646 & 5.42 $\pm$ 0.429 & 5.35 $\pm$ 0.443 & 5.38 $\pm$ 0.470 & 5.35 $\pm$ 0.463 & 5.33 $\pm$ 0.452 \\
\cline{1-9} \cline{2-9}
\multirow[c]{4}{*}{Ridge Regression} & \multirow[c]{2}{*}{DDPM} & Predicted & 8.24 $\pm$ 2.392 & 8.24 $\pm$ 2.392 & 8.24 $\pm$ 2.392 & 8.24 $\pm$ 2.392 & 8.24 $\pm$ 2.392 & 8.24 $\pm$ 2.392 \\
 &  & Measured & 8.24 $\pm$ 2.392 & 8.24 $\pm$ 2.392 & 8.31 $\pm$ 2.335 & 8.25 $\pm$ 2.388 & 7.79 $\pm$ 1.599 & 7.79 $\pm$ 1.599 \\
\cline{2-9}
 & \multirow[c]{2}{*}{SP-P} & Predicted & 5.57 $\pm$ 0.648 & 5.43 $\pm$ 0.432 & 5.35 $\pm$ 0.355 & 5.32 $\pm$ 0.332 & 5.30 $\pm$ 0.326 & 5.29 $\pm$ 0.323 \\
 &  & Measured & 5.57 $\pm$ 0.648 & 5.43 $\pm$ 0.432 & 5.35 $\pm$ 0.445 & 5.39 $\pm$ 0.472 & 5.35 $\pm$ 0.465 & 5.33 $\pm$ 0.454 \\
\cline{1-9} \cline{2-9}
\multirow[c]{4}{*}{1-NN} & \multirow[c]{2}{*}{DDPM} & Predicted & 9.01 $\pm$ 0.621 & 9.01 $\pm$ 0.621 & 9.01 $\pm$ 0.621 & 9.01 $\pm$ 0.621 & 9.01 $\pm$ 0.621 & 9.01 $\pm$ 0.621 \\
 &  & Measured & 9.01 $\pm$ 0.621 & 9.01 $\pm$ 0.621 & 8.57 $\pm$ 0.621 & 8.27 $\pm$ 0.123 & 7.72 $\pm$ 0.434 & 7.72 $\pm$ 0.434 \\
\cline{2-9}
 & \multirow[c]{2}{*}{SP-P} & Predicted & 9.52 $\pm$ 0.890 & 7.35 $\pm$ 0.764 & 6.26 $\pm$ 0.702 & 5.72 $\pm$ 0.670 & 5.45 $\pm$ 0.655 & 5.31 $\pm$ 0.647 \\
 &  & Measured & 9.52 $\pm$ 0.890 & 7.35 $\pm$ 0.764 & 6.21 $\pm$ 0.482 & 5.66 $\pm$ 0.514 & 5.30 $\pm$ 0.439 & 5.13 $\pm$ 0.479 \\
\cline{1-9} \cline{2-9}
\multirow[c]{4}{*}{5-NN} & \multirow[c]{2}{*}{DDPM} & Predicted & 5.76 $\pm$ 0.457 & 5.76 $\pm$ 0.457 & 5.76 $\pm$ 0.457 & 5.76 $\pm$ 0.457 & 5.76 $\pm$ 0.457 & 5.76 $\pm$ 0.457 \\
 &  & Measured & 5.76 $\pm$ 0.457 & 5.76 $\pm$ 0.457 & 5.71 $\pm$ 0.399 & 5.66 $\pm$ 0.493 & 5.56 $\pm$ 0.491 & 5.56 $\pm$ 0.491 \\
\cline{2-9}
 & \multirow[c]{2}{*}{SP-P} & Predicted & 6.32 $\pm$ 0.932 & 5.75 $\pm$ 0.704 & 5.46 $\pm$ 0.589 & 5.32 $\pm$ 0.532 & 5.25 $\pm$ 0.504 & 5.22 $\pm$ 0.489 \\
 &  & Measured & 6.32 $\pm$ 0.932 & 5.75 $\pm$ 0.704 & 5.42 $\pm$ 0.550 & 5.26 $\pm$ 0.539 & 5.18 $\pm$ 0.523 & 5.14 $\pm$ 0.513 \\
\cline{1-9} \cline{2-9}
\multirow[c]{4}{*}{Decision Tree} & \multirow[c]{2}{*}{DDPM} & Predicted & 9.17 $\pm$ 0.199 & 8.79 $\pm$ 0.289 & 8.60 $\pm$ 0.335 & 8.50 $\pm$ 0.358 & 8.45 $\pm$ 0.370 & 8.43 $\pm$ 0.375 \\
 &  & Measured & 9.17 $\pm$ 0.199 & 8.79 $\pm$ 0.289 & 8.19 $\pm$ 0.741 & 7.81 $\pm$ 0.509 & 7.17 $\pm$ 0.174 & 7.17 $\pm$ 0.194 \\
\cline{2-9}
 & \multirow[c]{2}{*}{SP-P} & Predicted & 9.37 $\pm$ 0.523 & 7.38 $\pm$ 0.418 & 6.38 $\pm$ 0.385 & 5.88 $\pm$ 0.375 & 5.64 $\pm$ 0.371 & 5.51 $\pm$ 0.370 \\
 &  & Measured & 9.37 $\pm$ 0.523 & 7.38 $\pm$ 0.418 & 6.05 $\pm$ 0.237 & 5.43 $\pm$ 0.165 & 5.07 $\pm$ 0.274 & 4.95 $\pm$ 0.348 \\
\cline{1-9} \cline{2-9}
\multirow[c]{4}{*}{Random Forest} & \multirow[c]{2}{*}{DDPM} & Predicted & 5.36 $\pm$ 0.372 & 5.34 $\pm$ 0.405 & 5.33 $\pm$ 0.422 & 5.33 $\pm$ 0.431 & 5.33 $\pm$ 0.435 & 5.33 $\pm$ 0.437 \\
 &  & Measured & 5.36 $\pm$ 0.372 & 5.34 $\pm$ 0.405 & 5.24 $\pm$ 0.361 & 5.21 $\pm$ 0.399 & 5.14 $\pm$ 0.360 & 5.13 $\pm$ 0.361 \\
\cline{2-9}
 & \multirow[c]{2}{*}{SP-P} & Predicted & 5.76 $\pm$ 0.378 & 5.40 $\pm$ 0.282 & 5.23 $\pm$ 0.235 & 5.14 $\pm$ 0.212 & 5.09 $\pm$ 0.201 & 5.07 $\pm$ 0.195 \\
 &  & Measured & 5.76 $\pm$ 0.378 & 5.40 $\pm$ 0.282 & 5.12 $\pm$ 0.268 & 4.96 $\pm$ 0.253 & 4.87 $\pm$ 0.276 & 4.85 $\pm$ 0.318 \\
\cline{1-9} \cline{2-9}
\multirow[c]{4}{*}{Gradient Boosting} & \multirow[c]{2}{*}{DDPM} & Predicted & 5.47 $\pm$ 0.506 & 5.47 $\pm$ 0.506 & 5.47 $\pm$ 0.506 & 5.47 $\pm$ 0.506 & 5.47 $\pm$ 0.506 & 5.47 $\pm$ 0.506 \\
 &  & Measured & 5.47 $\pm$ 0.506 & 5.47 $\pm$ 0.506 & 5.47 $\pm$ 0.503 & 5.45 $\pm$ 0.526 & 5.39 $\pm$ 0.509 & 5.39 $\pm$ 0.508 \\
\cline{2-9}
 & \multirow[c]{2}{*}{SP-P} & Predicted & 5.45 $\pm$ 0.336 & 5.25 $\pm$ 0.301 & 5.15 $\pm$ 0.303 & 5.11 $\pm$ 0.310 & 5.08 $\pm$ 0.314 & 5.07 $\pm$ 0.317 \\
 &  & Measured & 5.45 $\pm$ 0.336 & 5.25 $\pm$ 0.301 & 5.08 $\pm$ 0.294 & 4.99 $\pm$ 0.329 & 4.96 $\pm$ 0.324 & 4.96 $\pm$ 0.363 \\
\cline{1-9} \cline{2-9}
\multirow[c]{4}{*}{MLP} & \multirow[c]{2}{*}{DDPM} & Predicted & 5.06 $\pm$ 0.323 & 5.04 $\pm$ 0.335 & 5.03 $\pm$ 0.341 & 5.03 $\pm$ 0.345 & 5.02 $\pm$ 0.346 & 5.02 $\pm$ 0.347 \\
 &  & Measured & 5.06 $\pm$ 0.323 & 5.04 $\pm$ 0.335 & 5.00 $\pm$ 0.249 & 5.00 $\pm$ 0.273 & 4.92 $\pm$ 0.267 & 4.92 $\pm$ 0.280 \\
\cline{2-9}
 & \multirow[c]{2}{*}{SP-P} & Predicted & 6.02 $\pm$ 1.935 & 5.38 $\pm$ 1.075 & 5.06 $\pm$ 0.652 & 4.90 $\pm$ 0.449 & 4.82 $\pm$ 0.354 & 4.78 $\pm$ 0.310 \\
 &  & Measured & 6.02 $\pm$ 1.935 & 5.38 $\pm$ 1.075 & 4.96 $\pm$ 0.550 & 4.97 $\pm$ 0.570 & 4.84 $\pm$ 0.399 & 4.81 $\pm$ 0.399 \\
\cline{1-9} \cline{2-9}
\multirow[c]{4}{*}{SVM} & \multirow[c]{2}{*}{DDPM} & Predicted & 5.55 $\pm$ 0.592 & 5.55 $\pm$ 0.592 & 5.55 $\pm$ 0.592 & 5.55 $\pm$ 0.592 & 5.55 $\pm$ 0.592 & 5.55 $\pm$ 0.592 \\
 &  & Measured & 5.55 $\pm$ 0.592 & 5.55 $\pm$ 0.592 & 5.55 $\pm$ 0.586 & 5.54 $\pm$ 0.598 & 5.51 $\pm$ 0.610 & 5.51 $\pm$ 0.610 \\
\cline{2-9}
 & \multirow[c]{2}{*}{SP-P} & Predicted & 5.38 $\pm$ 0.515 & 5.35 $\pm$ 0.546 & 5.33 $\pm$ 0.567 & 5.33 $\pm$ 0.579 & 5.32 $\pm$ 0.585 & 5.32 $\pm$ 0.588 \\
 &  & Measured & 5.38 $\pm$ 0.515 & 5.35 $\pm$ 0.546 & 5.28 $\pm$ 0.499 & 5.28 $\pm$ 0.583 & 5.27 $\pm$ 0.604 & 5.26 $\pm$ 0.588 \\
\cline{1-9} \cline{2-9}
\bottomrule
\end{tabular}


==> figures/regression/california-housing-mse-est-table.tex <==
\begin{tabular}{lllllllll}
\toprule
 &  & m & 1 & 2 & 4 & 8 & 16 & 32 \\
Downstream & Generator & Predicted / Measured &  &  &  &  &  &  \\
\midrule
\multirow[c]{4}{*}{Linear Regression} & \multirow[c]{2}{*}{DDPM} & Predicted & 0.12 $\pm$ 0.004 & 0.12 $\pm$ 0.004 & 0.12 $\pm$ 0.004 & 0.12 $\pm$ 0.004 & 0.12 $\pm$ 0.004 & 0.12 $\pm$ 0.004 \\
 &  & Measured & 0.12 $\pm$ 0.004 & 0.12 $\pm$ 0.004 & 0.12 $\pm$ 0.003 & 0.12 $\pm$ 0.003 & 0.12 $\pm$ 0.003 & 0.12 $\pm$ 0.003 \\
\cline{2-9}
 & \multirow[c]{2}{*}{SP-P} & Predicted & 0.12 $\pm$ 0.001 & 0.11 $\pm$ 0.002 & 0.11 $\pm$ 0.002 & 0.11 $\pm$ 0.002 & 0.11 $\pm$ 0.002 & 0.11 $\pm$ 0.002 \\
 &  & Measured & 0.12 $\pm$ 0.001 & 0.11 $\pm$ 0.002 & 0.11 $\pm$ 0.002 & 0.11 $\pm$ 0.001 & 0.11 $\pm$ 0.002 & 0.11 $\pm$ 0.002 \\
\cline{1-9} \cline{2-9}
\multirow[c]{4}{*}{Ridge Regression} & \multirow[c]{2}{*}{DDPM} & Predicted & 0.12 $\pm$ 0.004 & 0.12 $\pm$ 0.004 & 0.12 $\pm$ 0.004 & 0.12 $\pm$ 0.004 & 0.12 $\pm$ 0.004 & 0.12 $\pm$ 0.004 \\
 &  & Measured & 0.12 $\pm$ 0.004 & 0.12 $\pm$ 0.004 & 0.12 $\pm$ 0.003 & 0.12 $\pm$ 0.003 & 0.12 $\pm$ 0.003 & 0.12 $\pm$ 0.003 \\
\cline{2-9}
 & \multirow[c]{2}{*}{SP-P} & Predicted & 0.12 $\pm$ 0.001 & 0.11 $\pm$ 0.002 & 0.11 $\pm$ 0.002 & 0.11 $\pm$ 0.002 & 0.11 $\pm$ 0.002 & 0.11 $\pm$ 0.002 \\
 &  & Measured & 0.12 $\pm$ 0.001 & 0.11 $\pm$ 0.002 & 0.11 $\pm$ 0.002 & 0.11 $\pm$ 0.001 & 0.11 $\pm$ 0.002 & 0.11 $\pm$ 0.002 \\
\cline{1-9} \cline{2-9}
\multirow[c]{4}{*}{1-NN} & \multirow[c]{2}{*}{DDPM} & Predicted & 0.14 $\pm$ 0.008 & 0.14 $\pm$ 0.008 & 0.14 $\pm$ 0.008 & 0.14 $\pm$ 0.008 & 0.14 $\pm$ 0.008 & 0.14 $\pm$ 0.008 \\
 &  & Measured & 0.14 $\pm$ 0.008 & 0.14 $\pm$ 0.008 & 0.12 $\pm$ 0.006 & 0.13 $\pm$ 0.007 & 0.12 $\pm$ 0.004 & 0.12 $\pm$ 0.004 \\
\cline{2-9}
 & \multirow[c]{2}{*}{SP-P} & Predicted & 0.16 $\pm$ 0.002 & 0.12 $\pm$ 0.002 & 0.09 $\pm$ 0.004 & 0.08 $\pm$ 0.004 & 0.07 $\pm$ 0.005 & 0.07 $\pm$ 0.005 \\
 &  & Measured & 0.16 $\pm$ 0.002 & 0.12 $\pm$ 0.002 & 0.09 $\pm$ 0.002 & 0.08 $\pm$ 0.001 & 0.08 $\pm$ 0.002 & 0.08 $\pm$ 0.001 \\
\cline{1-9} \cline{2-9}
\multirow[c]{4}{*}{5-NN} & \multirow[c]{2}{*}{DDPM} & Predicted & 0.09 $\pm$ 0.002 & 0.09 $\pm$ 0.002 & 0.09 $\pm$ 0.002 & 0.09 $\pm$ 0.002 & 0.09 $\pm$ 0.002 & 0.09 $\pm$ 0.002 \\
 &  & Measured & 0.09 $\pm$ 0.002 & 0.09 $\pm$ 0.002 & 0.09 $\pm$ 0.002 & 0.09 $\pm$ 0.002 & 0.09 $\pm$ 0.002 & 0.09 $\pm$ 0.002 \\
\cline{2-9}
 & \multirow[c]{2}{*}{SP-P} & Predicted & 0.10 $\pm$ 0.003 & 0.09 $\pm$ 0.001 & 0.08 $\pm$ 0.001 & 0.08 $\pm$ 0.001 & 0.08 $\pm$ 0.001 & 0.08 $\pm$ 0.001 \\
 &  & Measured & 0.10 $\pm$ 0.003 & 0.09 $\pm$ 0.001 & 0.08 $\pm$ 0.001 & 0.08 $\pm$ 0.001 & 0.08 $\pm$ 0.001 & 0.08 $\pm$ 0.001 \\
\cline{1-9} \cline{2-9}
\multirow[c]{4}{*}{Decision Tree} & \multirow[c]{2}{*}{DDPM} & Predicted & 0.13 $\pm$ 0.003 & 0.13 $\pm$ 0.004 & 0.13 $\pm$ 0.004 & 0.13 $\pm$ 0.005 & 0.13 $\pm$ 0.005 & 0.13 $\pm$ 0.005 \\
 &  & Measured & 0.13 $\pm$ 0.003 & 0.13 $\pm$ 0.004 & 0.10 $\pm$ 0.004 & 0.11 $\pm$ 0.006 & 0.10 $\pm$ 0.001 & 0.10 $\pm$ 0.002 \\
\cline{2-9}
 & \multirow[c]{2}{*}{SP-P} & Predicted & 0.15 $\pm$ 0.004 & 0.10 $\pm$ 0.004 & 0.08 $\pm$ 0.007 & 0.07 $\pm$ 0.009 & 0.06 $\pm$ 0.010 & 0.06 $\pm$ 0.010 \\
 &  & Measured & 0.15 $\pm$ 0.004 & 0.10 $\pm$ 0.004 & 0.08 $\pm$ 0.001 & 0.07 $\pm$ 0.001 & 0.07 $\pm$ 0.001 & 0.06 $\pm$ 0.001 \\
\cline{1-9} \cline{2-9}
\multirow[c]{4}{*}{Random Forest} & \multirow[c]{2}{*}{DDPM} & Predicted & 0.07 $\pm$ 0.002 & 0.07 $\pm$ 0.002 & 0.07 $\pm$ 0.002 & 0.07 $\pm$ 0.002 & 0.07 $\pm$ 0.002 & 0.07 $\pm$ 0.002 \\
 &  & Measured & 0.07 $\pm$ 0.002 & 0.07 $\pm$ 0.002 & 0.07 $\pm$ 0.001 & 0.07 $\pm$ 0.001 & 0.07 $\pm$ 0.001 & 0.07 $\pm$ 0.001 \\
\cline{2-9}
 & \multirow[c]{2}{*}{SP-P} & Predicted & 0.08 $\pm$ 0.002 & 0.07 $\pm$ 0.003 & 0.07 $\pm$ 0.004 & 0.06 $\pm$ 0.004 & 0.06 $\pm$ 0.005 & 0.06 $\pm$ 0.005 \\
 &  & Measured & 0.08 $\pm$ 0.002 & 0.07 $\pm$ 0.003 & 0.07 $\pm$ 0.002 & 0.06 $\pm$ 0.001 & 0.06 $\pm$ 0.001 & 0.06 $\pm$ 0.001 \\
\cline{1-9} \cline{2-9}
\multirow[c]{4}{*}{Gradient Boosting} & \multirow[c]{2}{*}{DDPM} & Predicted & 0.07 $\pm$ 0.002 & 0.07 $\pm$ 0.002 & 0.07 $\pm$ 0.002 & 0.07 $\pm$ 0.002 & 0.07 $\pm$ 0.002 & 0.07 $\pm$ 0.002 \\
 &  & Measured & 0.07 $\pm$ 0.002 & 0.07 $\pm$ 0.002 & 0.07 $\pm$ 0.002 & 0.07 $\pm$ 0.002 & 0.07 $\pm$ 0.002 & 0.07 $\pm$ 0.002 \\
\cline{2-9}
 & \multirow[c]{2}{*}{SP-P} & Predicted & 0.08 $\pm$ 0.002 & 0.07 $\pm$ 0.002 & 0.07 $\pm$ 0.002 & 0.07 $\pm$ 0.002 & 0.07 $\pm$ 0.002 & 0.07 $\pm$ 0.002 \\
 &  & Measured & 0.08 $\pm$ 0.002 & 0.07 $\pm$ 0.002 & 0.07 $\pm$ 0.001 & 0.07 $\pm$ 0.001 & 0.07 $\pm$ 0.001 & 0.07 $\pm$ 0.001 \\
\cline{1-9} \cline{2-9}
\multirow[c]{4}{*}{MLP} & \multirow[c]{2}{*}{DDPM} & Predicted & 0.07 $\pm$ 0.000 & 0.07 $\pm$ 0.001 & 0.07 $\pm$ 0.001 & 0.06 $\pm$ 0.001 & 0.06 $\pm$ 0.001 & 0.06 $\pm$ 0.001 \\
 &  & Measured & 0.07 $\pm$ 0.000 & 0.07 $\pm$ 0.001 & 0.07 $\pm$ 0.001 & 0.07 $\pm$ 0.001 & 0.06 $\pm$ 0.001 & 0.06 $\pm$ 0.001 \\
\cline{2-9}
 & \multirow[c]{2}{*}{SP-P} & Predicted & 0.08 $\pm$ 0.001 & 0.07 $\pm$ 0.002 & 0.07 $\pm$ 0.002 & 0.07 $\pm$ 0.003 & 0.07 $\pm$ 0.003 & 0.07 $\pm$ 0.003 \\
 &  & Measured & 0.08 $\pm$ 0.001 & 0.07 $\pm$ 0.002 & 0.07 $\pm$ 0.002 & 0.07 $\pm$ 0.001 & 0.07 $\pm$ 0.001 & 0.07 $\pm$ 0.001 \\
\cline{1-9} \cline{2-9}
\multirow[c]{4}{*}{SVM} & \multirow[c]{2}{*}{DDPM} & Predicted & 0.07 $\pm$ 0.001 & 0.07 $\pm$ 0.001 & 0.07 $\pm$ 0.001 & 0.07 $\pm$ 0.001 & 0.07 $\pm$ 0.001 & 0.07 $\pm$ 0.001 \\
 &  & Measured & 0.07 $\pm$ 0.001 & 0.07 $\pm$ 0.001 & 0.07 $\pm$ 0.001 & 0.07 $\pm$ 0.001 & 0.07 $\pm$ 0.001 & 0.07 $\pm$ 0.001 \\
\cline{2-9}
 & \multirow[c]{2}{*}{SP-P} & Predicted & 0.08 $\pm$ 0.001 & 0.07 $\pm$ 0.001 & 0.07 $\pm$ 0.002 & 0.07 $\pm$ 0.002 & 0.07 $\pm$ 0.002 & 0.07 $\pm$ 0.002 \\
 &  & Measured & 0.08 $\pm$ 0.001 & 0.07 $\pm$ 0.001 & 0.07 $\pm$ 0.001 & 0.07 $\pm$ 0.001 & 0.07 $\pm$ 0.001 & 0.07 $\pm$ 0.001 \\
\cline{1-9} \cline{2-9}
\bottomrule
\end{tabular}


==> figures/regression/insurance-mse-est-table.tex <==
\begin{tabular}{lllllllll}
\toprule
 &  & m & 1 & 2 & 4 & 8 & 16 & 32 \\
Downstream & Generator & Predicted / Measured &  &  &  &  &  &  \\
\midrule
\multirow[c]{4}{*}{Linear Regression} & \multirow[c]{2}{*}{DDPM} & Predicted & 0.25 $\pm$ 0.037 & 0.24 $\pm$ 0.039 & 0.23 $\pm$ 0.045 & 0.23 $\pm$ 0.048 & 0.22 $\pm$ 0.050 & 0.22 $\pm$ 0.051 \\
 &  & Measured & 0.25 $\pm$ 0.037 & 0.24 $\pm$ 0.039 & 0.23 $\pm$ 0.030 & 0.23 $\pm$ 0.023 & 0.23 $\pm$ 0.020 & 0.23 $\pm$ 0.021 \\
\cline{2-9}
 & \multirow[c]{2}{*}{SP-P} & Predicted & 0.20 $\pm$ 0.009 & 0.20 $\pm$ 0.009 & 0.20 $\pm$ 0.010 & 0.20 $\pm$ 0.010 & 0.20 $\pm$ 0.010 & 0.20 $\pm$ 0.010 \\
 &  & Measured & 0.20 $\pm$ 0.009 & 0.20 $\pm$ 0.009 & 0.20 $\pm$ 0.008 & 0.20 $\pm$ 0.006 & 0.20 $\pm$ 0.006 & 0.20 $\pm$ 0.006 \\
\cline{1-9} \cline{2-9}
\multirow[c]{4}{*}{Ridge Regression} & \multirow[c]{2}{*}{DDPM} & Predicted & 0.25 $\pm$ 0.037 & 0.24 $\pm$ 0.039 & 0.23 $\pm$ 0.045 & 0.23 $\pm$ 0.048 & 0.22 $\pm$ 0.050 & 0.22 $\pm$ 0.051 \\
 &  & Measured & 0.25 $\pm$ 0.037 & 0.24 $\pm$ 0.039 & 0.23 $\pm$ 0.031 & 0.23 $\pm$ 0.023 & 0.23 $\pm$ 0.021 & 0.23 $\pm$ 0.021 \\
\cline{2-9}
 & \multirow[c]{2}{*}{SP-P} & Predicted & 0.20 $\pm$ 0.009 & 0.20 $\pm$ 0.010 & 0.20 $\pm$ 0.010 & 0.20 $\pm$ 0.010 & 0.20 $\pm$ 0.010 & 0.20 $\pm$ 0.010 \\
 &  & Measured & 0.20 $\pm$ 0.009 & 0.20 $\pm$ 0.010 & 0.20 $\pm$ 0.008 & 0.20 $\pm$ 0.007 & 0.20 $\pm$ 0.006 & 0.20 $\pm$ 0.006 \\
\cline{1-9} \cline{2-9}
\multirow[c]{4}{*}{1-NN} & \multirow[c]{2}{*}{DDPM} & Predicted & 0.40 $\pm$ 0.076 & 0.37 $\pm$ 0.104 & 0.36 $\pm$ 0.124 & 0.35 $\pm$ 0.134 & 0.34 $\pm$ 0.139 & 0.34 $\pm$ 0.142 \\
 &  & Measured & 0.40 $\pm$ 0.076 & 0.37 $\pm$ 0.104 & 0.34 $\pm$ 0.056 & 0.33 $\pm$ 0.042 & 0.34 $\pm$ 0.040 & 0.34 $\pm$ 0.040 \\
\cline{2-9}
 & \multirow[c]{2}{*}{SP-P} & Predicted & 0.29 $\pm$ 0.063 & 0.20 $\pm$ 0.012 & 0.16 $\pm$ 0.015 & 0.14 $\pm$ 0.028 & 0.13 $\pm$ 0.034 & 0.12 $\pm$ 0.037 \\
 &  & Measured & 0.29 $\pm$ 0.063 & 0.20 $\pm$ 0.012 & 0.17 $\pm$ 0.015 & 0.15 $\pm$ 0.009 & 0.15 $\pm$ 0.006 & 0.14 $\pm$ 0.002 \\
\cline{1-9} \cline{2-9}
\multirow[c]{4}{*}{5-NN} & \multirow[c]{2}{*}{DDPM} & Predicted & 0.23 $\pm$ 0.031 & 0.21 $\pm$ 0.031 & 0.21 $\pm$ 0.039 & 0.20 $\pm$ 0.044 & 0.20 $\pm$ 0.047 & 0.20 $\pm$ 0.048 \\
 &  & Measured & 0.23 $\pm$ 0.031 & 0.21 $\pm$ 0.031 & 0.21 $\pm$ 0.017 & 0.20 $\pm$ 0.009 & 0.20 $\pm$ 0.014 & 0.21 $\pm$ 0.017 \\
\cline{2-9}
 & \multirow[c]{2}{*}{SP-P} & Predicted & 0.19 $\pm$ 0.014 & 0.16 $\pm$ 0.007 & 0.15 $\pm$ 0.004 & 0.14 $\pm$ 0.004 & 0.14 $\pm$ 0.004 & 0.14 $\pm$ 0.004 \\
 &  & Measured & 0.19 $\pm$ 0.014 & 0.16 $\pm$ 0.007 & 0.15 $\pm$ 0.008 & 0.15 $\pm$ 0.005 & 0.15 $\pm$ 0.005 & 0.14 $\pm$ 0.003 \\
\cline{1-9} \cline{2-9}
\multirow[c]{4}{*}{Decision Tree} & \multirow[c]{2}{*}{DDPM} & Predicted & 0.38 $\pm$ 0.074 & 0.34 $\pm$ 0.110 & 0.32 $\pm$ 0.134 & 0.31 $\pm$ 0.147 & 0.31 $\pm$ 0.154 & 0.30 $\pm$ 0.157 \\
 &  & Measured & 0.38 $\pm$ 0.074 & 0.34 $\pm$ 0.110 & 0.32 $\pm$ 0.075 & 0.31 $\pm$ 0.071 & 0.32 $\pm$ 0.070 & 0.33 $\pm$ 0.069 \\
\cline{2-9}
 & \multirow[c]{2}{*}{SP-P} & Predicted & 0.26 $\pm$ 0.011 & 0.21 $\pm$ 0.012 & 0.18 $\pm$ 0.016 & 0.16 $\pm$ 0.019 & 0.16 $\pm$ 0.020 & 0.15 $\pm$ 0.021 \\
 &  & Measured & 0.26 $\pm$ 0.011 & 0.21 $\pm$ 0.012 & 0.17 $\pm$ 0.003 & 0.16 $\pm$ 0.002 & 0.15 $\pm$ 0.007 & 0.14 $\pm$ 0.007 \\
\cline{1-9} \cline{2-9}
\multirow[c]{4}{*}{Random Forest} & \multirow[c]{2}{*}{DDPM} & Predicted & 0.22 $\pm$ 0.015 & 0.20 $\pm$ 0.028 & 0.19 $\pm$ 0.038 & 0.19 $\pm$ 0.043 & 0.19 $\pm$ 0.046 & 0.19 $\pm$ 0.047 \\
 &  & Measured & 0.22 $\pm$ 0.015 & 0.20 $\pm$ 0.028 & 0.19 $\pm$ 0.015 & 0.19 $\pm$ 0.013 & 0.19 $\pm$ 0.009 & 0.19 $\pm$ 0.010 \\
\cline{2-9}
 & \multirow[c]{2}{*}{SP-P} & Predicted & 0.18 $\pm$ 0.023 & 0.16 $\pm$ 0.019 & 0.15 $\pm$ 0.021 & 0.15 $\pm$ 0.023 & 0.15 $\pm$ 0.024 & 0.14 $\pm$ 0.024 \\
 &  & Measured & 0.18 $\pm$ 0.023 & 0.16 $\pm$ 0.019 & 0.15 $\pm$ 0.007 & 0.14 $\pm$ 0.006 & 0.14 $\pm$ 0.008 & 0.14 $\pm$ 0.007 \\
\cline{1-9} \cline{2-9}
\multirow[c]{4}{*}{Gradient Boosting} & \multirow[c]{2}{*}{DDPM} & Predicted & 0.18 $\pm$ 0.017 & 0.17 $\pm$ 0.011 & 0.17 $\pm$ 0.014 & 0.17 $\pm$ 0.017 & 0.17 $\pm$ 0.018 & 0.17 $\pm$ 0.019 \\
 &  & Measured & 0.18 $\pm$ 0.017 & 0.17 $\pm$ 0.011 & 0.17 $\pm$ 0.004 & 0.17 $\pm$ 0.005 & 0.17 $\pm$ 0.013 & 0.17 $\pm$ 0.016 \\
\cline{2-9}
 & \multirow[c]{2}{*}{SP-P} & Predicted & 0.16 $\pm$ 0.009 & 0.15 $\pm$ 0.009 & 0.14 $\pm$ 0.012 & 0.14 $\pm$ 0.014 & 0.14 $\pm$ 0.015 & 0.14 $\pm$ 0.015 \\
 &  & Measured & 0.16 $\pm$ 0.009 & 0.15 $\pm$ 0.009 & 0.14 $\pm$ 0.007 & 0.14 $\pm$ 0.009 & 0.14 $\pm$ 0.010 & 0.13 $\pm$ 0.009 \\
\cline{1-9} \cline{2-9}
\multirow[c]{4}{*}{MLP} & \multirow[c]{2}{*}{DDPM} & Predicted & 0.23 $\pm$ 0.010 & 0.23 $\pm$ 0.008 & 0.22 $\pm$ 0.007 & 0.22 $\pm$ 0.007 & 0.22 $\pm$ 0.008 & 0.22 $\pm$ 0.008 \\
 &  & Measured & 0.23 $\pm$ 0.010 & 0.23 $\pm$ 0.008 & 0.21 $\pm$ 0.008 & 0.20 $\pm$ 0.009 & 0.20 $\pm$ 0.013 & 0.20 $\pm$ 0.014 \\
\cline{2-9}
 & \multirow[c]{2}{*}{SP-P} & Predicted & 0.16 $\pm$ 0.009 & 0.16 $\pm$ 0.011 & 0.15 $\pm$ 0.012 & 0.15 $\pm$ 0.013 & 0.15 $\pm$ 0.013 & 0.15 $\pm$ 0.014 \\
 &  & Measured & 0.16 $\pm$ 0.009 & 0.16 $\pm$ 0.011 & 0.15 $\pm$ 0.009 & 0.15 $\pm$ 0.009 & 0.15 $\pm$ 0.011 & 0.15 $\pm$ 0.012 \\
\cline{1-9} \cline{2-9}
\multirow[c]{4}{*}{SVM} & \multirow[c]{2}{*}{DDPM} & Predicted & 0.18 $\pm$ 0.018 & 0.17 $\pm$ 0.023 & 0.16 $\pm$ 0.028 & 0.16 $\pm$ 0.031 & 0.16 $\pm$ 0.032 & 0.16 $\pm$ 0.033 \\
 &  & Measured & 0.18 $\pm$ 0.018 & 0.17 $\pm$ 0.023 & 0.16 $\pm$ 0.015 & 0.16 $\pm$ 0.010 & 0.16 $\pm$ 0.004 & 0.16 $\pm$ 0.004 \\
\cline{2-9}
 & \multirow[c]{2}{*}{SP-P} & Predicted & 0.15 $\pm$ 0.015 & 0.14 $\pm$ 0.014 & 0.14 $\pm$ 0.015 & 0.14 $\pm$ 0.015 & 0.14 $\pm$ 0.015 & 0.14 $\pm$ 0.015 \\
 &  & Measured & 0.15 $\pm$ 0.015 & 0.14 $\pm$ 0.014 & 0.14 $\pm$ 0.015 & 0.14 $\pm$ 0.015 & 0.14 $\pm$ 0.015 & 0.14 $\pm$ 0.014 \\
\cline{1-9} \cline{2-9}
\bottomrule
\end{tabular}

